SHOPPER: A Probabilistic Model of Consumer Choice with Substitutes and Complements

We develop SHOPPER, a sequential probabilistic model of shopping data. SHOPPER uses interpretable components to model the forces that drive how a customer chooses products; in particular, we designed SHOPPER to capture how items interact with other items. We develop an efficient posterior inference algorithm to estimate these forces from large-scale data, and we analyze a large dataset from a major chain grocery store. We are interested in answering counterfactual queries about changes in prices. We found that SHOPPER provides accurate predictions even under price interventions, and that it helps identify complementary and substitutable pairs of products.

==> sec_background.tex <==
% !TEX root = main.tex
\section{Background: Exponential Family Embeddings}
\label{sec:background}

Exponential family embeddings \citep{Rudolph2016} extend the main idea behind word embeddings to other data beyond text. For that, they use tools from exponential families \citep{Brown1986} and generalized linear models \citep{McCullagh1989}.

Exponential family embeddings are conditionally specified models. They focus on estimating the probability of a data point given other data points in the \emph{context}. In the case of item embeddings, the context is defined as the set of all the items in the shopping basket, except for the target one.

Formally, we use $y_{ti}\in\{0,1\}$ to denote whether item was $i$ purchased at the $t$-th trip to the supermarket. For each observation $y_{ti}$, the context $\Ccal_{ti}$ is defined as the set of indices of all items purchased at that trip, excluding $i$, i.e., $\Ccal_{ti}=\{j: y_{tj}=1, j\neq i\}$.

Exponential family embeddings model the data using a set of \emph{embedding vectors} $\brho$ and \emph{context vectors} $\balpha$. In item embeddings, we have an embedding vector $\brho_i$ and a context vector $\balpha_i$ for each item $i\in\{1,2,\ldots,I\}$. Embedding vectors model the probability of an item given its context, whereas context vectors model how an item in the context affects the probability of other items. We make this precise below.

The embedding vectors determine the conditional distribution of a data point $y_{ti}$ given its context through an exponential family distribution. For binary data, a natural choice is the Bernoulli distribution,
\begin{equation}\label{eq:p_y}
	p\left(y_{ti}\g \{y_{tj}\}_{j\in \Ccal_{ti}} \right) = \textrm{Bernoulli}\left(
	\sigma(\eta_{ti})
	\right),
\end{equation}
where $\eta_{ti}$ is the natural parameter of the Bernoulli, which relates to the mean parameter through the sigmoid function, $\sigma(\eta) = 1/(1+e^{-\eta})$. The natural parameter is chosen as the inner product between the embedding vector and a weighted average of the context vectors, 
\begin{equation}\label{eq:eta_pemb}
	\eta_{ti} = \brho_i^\top \frac{1}{N_{ti}} \sum_{j=1}^{I} y_{tj}\balpha_j = \brho_i^\top \frac{1}{N_{ti}} \sum_{j\in \Ccal_{ti}} \balpha_j,
\end{equation}
where $N_{ti}=\sum_{j\in\Ccal_{ti}}y_{tj}$ is the number of items purchased at trip $t$, excluding item $i$ \citep{Rudolph2016}.

With these ingredients, we now form the objective function of the resulting Bernoulli exponential family embedding model. We combine the log-probabilities in \Cref{eq:p_y}, together with regularization terms,
\begin{equation}\label{eq:objective_pemb}
	\begin{split}
		\Lcal &= \Lcal_{\textrm{reg}} + \sum_{t=1}^{T}\sum_{i=1}^{I}  \log p\left(y_{ti}\g \{y_{tj}\}_{j\in \Ccal_{ti}} \right) \\
		&= \Lcal_{\textrm{reg}} + \sum_{t=1}^{T}\sum_{i=1}^{I} \big( y_{ti}\eta_{ti}-\log(1+e^{\eta_{ti}}) \big),
	\end{split}
\end{equation}
where $\Lcal_{\textrm{reg}}$ denotes an $\ell_2$ regularization term over each $\brho_i$ and $\balpha_i$. Fitting a Bernoulli exponential family embedding model involves maximizing $\Lcal$ with respect to the embedding and context vectors.

Moreover, \citet{Rudolph2016} artificially downweigh the contribution of the zeros in the objective function in \Cref{eq:objective_pemb}. This improves performance, as it allows the model to focus on the ``positive signal'' of the actual purchases \citep{Hu2008,Liang2016exposure}.


